Spillover of Antisocial Behavior from Fringe Platforms: The Unintended Consequences of Community Banning

Online platforms face pressure to keep their communities civil and respectful. Thus, the bannings of problematic online communities from mainstream platforms like Reddit and Facebook are often met with enthusiastic public reactions. However, this policy can lead users to migrate to alternative fringe platforms with lower moderation standards and where antisocial behaviors like trolling and harassment are widely accepted. As users of these communities often remain co-active across mainstream and fringe platforms, antisocial behaviors may spill over onto the mainstream platform. We study this possible spillover by analyzing around 70,000 users from three banned communities that migrated to fringe platforms: r/The_Donald, r/GenderCritical, and r/Incels. Using a difference-in-differences design, we contrast co-active users with matched counterparts to estimate the causal effect of fringe platform participation on users' antisocial behavior on Reddit. Our results show that participating in the fringe communities increases users' toxicity on Reddit (as measured by Perspective API) and involvement with subreddits similar to the banned community -- which often also breach platform norms. The effect intensifies with time and exposure to the fringe platform. In short, we find evidence for a spillover of antisocial behavior from fringe platforms onto Reddit via co-participation.

==> tabs/table_did_regr.tex <==
\sisetup{
  input-symbols         = (),
  table-format          = -1.5,
  table-space-text-post = ***,
  table-align-text-post = false,
  group-digits          = true,
  round-mode=places,
  round-precision=3
}
\begin{table*}
\tiny
\centering
\begin{tabular}{l D{.}{.}{2.6} D{.}{.}{2.6} D{.}{.}{2.6} D{.}{.}{2.8} D{.}{.}{2.6} D{.}{.}{2.6}}
\toprule
& \multicolumn{2}{c}{The Donald} & \multicolumn{2}{c}{Gender Critical} & \multicolumn{2}{c}{Incels}\\
\midrule
 & \mc{Toxicity} & \mc{Engagement} & \mc{Toxicity} & \mc{Engagement} & \mc{Toxicity} & \mc{Engagement} \\
\midrule
Coactive         & -0.560       & 0.185       & 0.025        & -2.041        & 2.567        & -3.554       \\
                         & (0.423)      & (0.737)     & (1.957)      & (2.343)       & (1.604)      & (3.594)      \\
Coactive:Period1 & 2.021^{**}   & 2.926^{**}  & 5.813^{*}    & 7.288^{\cdot} & 7.436^{***}  & 8.254        \\
                         & (0.629)      & (1.110)     & (2.335)      & (4.156)       & (1.900)      & (5.096)      \\
Coactive:Period2 & 1.876^{**}   & 1.348       & 6.236^{*}    & 7.782^{\cdot} & 7.850^{***}  & 16.378^{**}  \\
                         & (0.665)      & (1.116)     & (2.458)      & (3.976)       & (2.031)      & (5.752)      \\
Coactive:Period3 & 3.649^{***}  & 7.046^{***} & 9.400^{***}  & 1.778         & 8.923^{***}  & 14.669^{*}   \\
                         & (0.683)      & (1.222)     & (2.115)      & (4.265)       & (1.941)      & (6.001)      \\
Coactive:Period4 & 7.009^{***}  & 6.851^{***} & 10.250^{***} & 6.699         & 9.055^{***}  & 24.527^{***} \\
                         & (0.674)      & (1.254)     & (2.064)      & (4.714)       & (1.736)      & (6.571)      \\
\midrule
\multicolumn{7}{l}{\scriptsize{\emph{Controls}}}\\
\midrule
(Intercept)              & 13.500^{***} & 8.854^{***} & 16.664^{***} & 9.047^{***}   & 20.584^{***} & 22.250^{***} \\
                         & (0.301)      & (0.517)     & (1.267)      & (1.156)       & (1.112)      & (2.757)      \\
Period & \mc{Yes} & \mc{Yes}& \mc{Yes}& \mc{Yes}& \mc{Yes}& \mc{Yes}\\
\midrule
R$^2$                    & 0.088        & 0.034       & 0.084        & 0.019         & 0.078        & 0.120         \\
Adj. R$^2$               & 0.087        & 0.034       & 0.079        & 0.013         & 0.075        & 0.117         \\
Num. obs.                & 23158        & 27287       & 1783         & 1661          & 3129         & 2686          \\
\bottomrule
\multicolumn{7}{l}{\scriptsize{$^{***}p<0.001$; $^{**}p<0.01$; $^{*}p<0.05$; $^{\cdot}p<0.1$}}
\end{tabular}
\caption{Statistical models}
\label{table:coefficients}
\end{table*}


==> tabs/table_did_regr_fixed_effects.tex <==
\begin{table*}[t!]
\small
\centering
\begin{tabular}{l D{.}{.}{2.6} D{.}{.}{2.6} D{.}{.}{2.6} D{.}{.}{2.8} D{.}{.}{2.6} D{.}{.}{2.6}}
\toprule
\multicolumn{7}{c}{DiD Analysis (users fixed effects)}\\
\midrule
& \multicolumn{2}{c}{r/The\_Donald} & \multicolumn{2}{c}{r/GenderCritical} & \multicolumn{2}{c}{r/Incels}\\
\midrule
 & \mc{Toxicity} & \mc{Engagement} & \mc{Toxicity} & \mc{Engagement} & \mc{Toxicity} & \mc{Engagement} \\
\midrule
Coactive         & 0.625       & 92.301^{***} & -2.372       & -2.449   & -17.974      & 9.998        \\
                         & (7.177)     & (6.480)      & (4.273)      & (11.701) & (11.142)     & (19.095)     \\
Coactive:Period1 & 2.302^{***} & 3.668^{***}  & 7.748^{***}  & 2.039    & 8.270^{***}  & 4.292        \\
                         & (0.549)     & (0.764)      & (1.810)      & (3.339)  & (1.658)      & (3.826)      \\
Coactive:Period2 & 1.737^{**}  & 2.518^{**}   & 6.186^{***}  & 4.227    & 7.050^{***}  & 11.910^{**}  \\
                         & (0.552)     & (0.782)      & (1.748)      & (3.362)  & (1.677)      & (4.031)      \\
Coactive:Period3 & 3.046^{***} & 7.825^{***}  & 9.001^{***}  & -3.050   & 7.481^{***}  & 8.201^{*}    \\
                         & (0.564)     & (0.801)      & (1.763)      & (3.320)  & (1.698)      & (4.010)      \\
Coactive:Period4 & 6.644^{***} & 8.196^{***}  & 10.333^{***} & 3.186    & 7.303^{***}  & 18.267^{***} \\
                         & (0.572)     & (0.816)      & (1.782)      & (3.555)  & (1.634)      & (4.111)      \\
\midrule
\multicolumn{7}{l}{\scriptsize{\emph{Controls}}}\\
\midrule
(Intercept)              & 14.260^{*}  & -5.927       & 16.394^{***} & 2.909    & 34.919^{***} & 16.667       \\
                         & (6.417)     & (4.582)      & (3.218)      & (10.486) & (9.934)      & (16.684)     \\
Period & \mc{Yes} & \mc{Yes}& \mc{Yes}& \mc{Yes}& \mc{Yes}& \mc{Yes}\\
User Fixed Eff. & \mc{Yes} & \mc{Yes} & \mc{Yes} & \mc{Yes} & \mc{Yes} & \mc{Yes}\\
\midrule
R$^2$                    & 0.351       & 0.485        & 0.391        & 0.582    & 0.426        & 0.532        \\
Adj. R$^2$               & 0.291       & 0.448        & 0.341        & 0.365    & 0.359        & 0.474        \\
Num. obs.                & 23158       & 27287        & 1783         & 1661     & 3129         & 2686         \\
\bottomrule
\multicolumn{7}{l}{\scriptsize{$^{***}p<0.001$; $^{**}p<0.01$; $^{*}p<0.05$; $^{\cdot}p<0.1$}}
\end{tabular}
\caption{Supplementary regression table. Coefficient estimates and standard errors for the divergence analysis inclusive of users fixed effect. The inclusion of fixed effects mitigates possible omitted variable biases. The results are consistent with those of \cref{tab:predictors}.}
\label{tab:did_fe}
\end{table*}

